Neuro-Symbolic Continual Learning: Knowledge, Reasoning Shortcuts and Concept Rehearsal

We introduce Neuro-Symbolic Continual Learning, where a model has to solve a sequence of neuro-symbolic tasks, that is, it has to map sub-symbolic inputs to high-level concepts and compute predictions by reasoning consistently with prior knowledge. Our key observation is that neuro-symbolic tasks, although different, often share concepts whose semantics remains stable over time. Traditional approaches fall short: existing continual strategies ignore knowledge altogether, while stock neuro-symbolic architectures suffer from catastrophic forgetting. We show that leveraging prior knowledge by combining neuro-symbolic architectures with continual strategies does help avoid catastrophic forgetting, but also that doing so can yield models affected by reasoning shortcuts. These undermine the semantics of the acquired concepts, even when detailed prior knowledge is provided upfront and inference is exact, and in turn continual performance. To overcome these issues, we introduce COOL, a COncept-level cOntinual Learning strategy tailored for neuro-symbolic continual problems that acquires high-quality concepts and remembers them over time. Our experiments on three novel benchmarks highlights how COOL attains sustained high performance on neuro-symbolic continual learning tasks in which other strategies fail.

==> tables/CBM-vs-NeSy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{llcccccc}
                                                 & {\sc Strategy}       & TIL ($\uparrow$)    & CTIL ($\uparrow$)   & CIL ($\uparrow$)    & CCIL($\uparrow$)    & BWT ($\uparrow$)      & FWT ($\uparrow$) \\ \cmidrule{2-8}
\multirow{8}{*}{\rotatebox{90}{\sc CBM}}         & \restart    & $45.45$ $\pm$ 0.7     & 43.94 $\pm$ 0.25    & 11.31 $\pm$ 0.09    & 30.58 $\pm$ 0.06    & -97.97 $\pm$ 0.12     & 6.96 $\pm$ 0.77  \\
                                                 & \naive      & 44.08 $\pm$ 4.6     & 66.49 $\pm$ 5.89    & 17.42 $\pm$ 2.0     & 37.33 $\pm$ 3.68    & -91.52 $\pm$ 2.19     & 11.65 $\pm$ 2.3  \\
                                                 & \er         & 80.58 $\pm$ 4.64    & 88.45 $\pm$ 2.87    & 47.6 $\pm$ 6.26     & 68.62 $\pm$ 5.0     & -57.6 $\pm$ 7.09      & 43.85 $\pm$ 5.38 \\
                                                 & \erace      & 91.46 $\pm$ 1.0     & 92.24 $\pm$ 0.53    & 52.0 $\pm$ 1.43     & 77.11 $\pm$ 1.76    &\bf -20.71 $\pm$ 2.81     & 64.69 $\pm$ 5.1  \\
                                                 & \der        & 78.34 $\pm$ 8.74    & 88.06 $\pm$ 3.66    & 39.71 $\pm$ 7.48    & 67.39 $\pm$ 9.25    & -66.41 $\pm$ 8.38     & 36.28 $\pm$ 6.43 \\
                                                 & \derpp      & 81.64 $\pm$ 6.68    & 87.11 $\pm$ 3.6     & 46.22 $\pm$ 8.16    & 67.63 $\pm$ 7.78    & -59.17 $\pm$ 9.18     & 45.19 $\pm$ 8.52 \\
                                                 & \mer        &\bf 92.65 $\pm$ 3.37 &\bf 92.87 $\pm$ 1.21 &\bf 72.14 $\pm$ 4.74 &\bf 78.95 $\pm$ 4.65 & -28.96 $\pm$ 5.3      &\bf 74.13 $\pm$ 5.19 \\
                                                 & \methoder   & 82.74 $\pm$ 3.08    & 91.48 $\pm$ 2.52    & 48.69 $\pm$ 3.82    & 78.09 $\pm$ 3.49    & -56.4 $\pm$ 4.3       & 47.64 $\pm$ 3.67 \\ \cmidrule{2-8}
\multirow{9}{*}{\rotatebox{90}{\sc DeepProbLog}} & \restart    & 23.23 $\pm$ 0.45    & 10.83 $\pm$ 0.97    & 9.4 $\pm$ 0.13      & 0.14 $\pm$ 0.01     & -72.83 $\pm$ 1.7      & 7.3 $\pm$ 0.83   \\
                                                 & \naive      & 52.49 $\pm$ 8.74    & 17.1 $\pm$ 1.39     & 4.74 $\pm$ 0.49     & 12.46 $\pm$ 0.96    &\underline{-11.53 $\pm$ 11.49} & 6.45 $\pm$ 7.96  \\
                                                 & \er         & 93.53 $\pm$ 1.71    & 94.33 $\pm$ 0.55    & 65.28 $\pm$ 2.93    & 79.59 $\pm$ 2.15    & -28.82 $\pm$ 3.07     & 14.9 $\pm$ 6.16  \\
                                                 & \erace      & 90.42 $\pm$ 4.02    & 91.4 $\pm$ 3.24     & 58.48 $\pm$ 6.6     & 74.15 $\pm$ 5.54    & -37.14 $\pm$ 5.16     & 24.15 $\pm$ 2.94 \\
                                                 & \der        & 96.04 $\pm$ 1.03    & 94.41 $\pm$ 1.45    & 69.44 $\pm$ 2.98    & 82.33 $\pm$ 2.07    & -27.48 $\pm$ 3.48     & 26.62 $\pm$ 3.01 \\
                                                 & \derpp      & 94.27 $\pm$ 1.79    & 93.09 $\pm$ 3.19    & 66.43 $\pm$ 5.7     & 80.27 $\pm$ 3.91    & -30.46 $\pm$ 5.74     & 23.64 $\pm$ 2.09 \\
                                                 & \mer        & 96.73 $\pm$ 0.32    & 95.02 $\pm$ 0.39    & 72.3 $\pm$ 3.35     & 84.66 $\pm$ 2.12    & -26.79 $\pm$ 3.89     & 82.03 $\pm$ 1.73 \\
                                                 & \method     &\bf 98.59 $\pm$ 0.19 &\bf 96.93 $\pm$ 0.24 &\bf 79.39 $\pm$ 2.52 &\bf 88.9 $\pm$ 1.47  & -21.0 $\pm$ 2.85      &\bf 86.22 $\pm$ 0.45 \\
                                                 & \methoder   & 97.95 $\pm$ 0.2     & 96.11 $\pm$ 0.2     & 78.35 $\pm$ 1.04    & 88.39 $\pm$ 0.67    &\bf -19.9 $\pm$ 1.3    & 85.18 $\pm$ 0.49 \\
\cmidrule{2-8}
\end{tabular}

==> tables/CLE4VR_with_sup.tex <==
\begin{tabular}{lcccccc}
   & \multicolumn{2}{c}{Supervision on $\vC$ = 0\%} & \multicolumn{2}{c}{Supervision on $\vC$ = 1\%}  & \multicolumn{2}{c}{Supervision on $\vC$ = 10\%}               \\
\sc Strategy& Class-IL ($\vY$)    & Class-IL ($\vC$)    & Class-IL ($\vY$)     & Class-IL ($\vC$)     & Class-IL ($\vY$)    & Class-IL ($\vC$)        \\ \cmidrule{1-7}
\naive      & 44.87 $\pm$ 0.66    & 9.15 $\pm$ 1.22     & 42.58 $\pm$ 2.71     & 19.57 $\pm$ 2.38     & 39.95 $\pm$ 1.64    & 17.86 $\pm$ 0.01 \\
\restart    & 39.07 $\pm$ 0.85    & 10.5 $\pm$ 1.43     & 39.33 $\pm$ 1.33     & 17.83 $\pm$ 0.11     & 39.15 $\pm$ 1.05    & 17.86 $\pm$ 0.01 \\
\er         &\bf 85.07 $\pm$ 0.49 &\bf 10.37 $\pm$ 5.07 & 69.28 $\pm$ 8.05     & 20.25 $\pm$ 3.66     & 66.86 $\pm$ 8.39    & 18.27 $\pm$ 1.29 \\
\er\_ace    & 84.9 $\pm$ 0.43     & 9.07 $\pm$ 5.52     & 77.51 $\pm$ 4.58     & 24.36 $\pm$ 4.83     & 78.26 $\pm$ 2.91    & 17.89 $\pm$ 0.07 \\
\der        & 76.93 $\pm$ 2.0     & 8.48 $\pm$ 3.32     & 69.92 $\pm$ 7.15     & 18.83 $\pm$ 1.84     & 72.71 $\pm$ 6.63    & 18.97 $\pm$ 1.91 \\
\derpp      &\bf 84.93 $\pm$ 0.85 &\bf 10.6 $\pm$ 4.48  & 79.41 $\pm$ 3.04     & 22.3 $\pm$ 4.28      & 79.21 $\pm$ 3.29    & 20.19 $\pm$ 3.77 \\
\method     & 53.6 $\pm$ 8.13     & 9.73 $\pm$ 1.79     & 74.65 $\pm$ 1.93     & 85.39 $\pm$ 1.66     & 83.37 $\pm$ 0.83    & 87.61 $\pm$ 0.2  \\
\methoder   & 70.75 $\pm$ 5.74    & 8.45 $\pm$ 4.45     & \bf 81.69 $\pm$ 1.6  &\bf 86.59 $\pm$ 2.17  &\bf 85.04 $\pm$ 0.43 &\bf 87.92 $\pm$ 0.11 \\ \cmidrule{1-7}
\end{tabular}


==> tables/SHORTCUT-MNIST.tex <==
\begin{tabular}{llccccccccccccc}
\sc Strategy & Class-IL ($\vY$)  & Class-IL ($\vC$)  & OOD ($\vY$)      & OOD ($\vC$)       &  & Class-IL ($\vY$)  & Class-IL ($\vC$) & OOD ($\vY$)      & OOD ($\vC$)       &  & Class-IL ($\vY$) & Class-IL ($\vC$) & OOD ($\vY$)      & OOD ($\vC$)      \\
\method  & 38.76 $\pm$ 26.25 & 24.08 $\pm$ 18.14 & 4.85 $\pm$ 2.02  & 23.61 $\pm$ 17.77 &  & 67.9 $\pm$ 1.98   & 77.67 $\pm$ 1.9  & 53.28 $\pm$ 3.89 & 74.65 $\pm$ 2.49  &  & 70.72 $\pm$ 2.13 & 80.23 $\pm$ 1.93 & 57.05 $\pm$ 3.95 & 76.8 $\pm$ 2.4   \\
\der     & 41.36 $\pm$ 13.06 & 19.57 $\pm$ 17.41 & 7.88 $\pm$ 1.73  & 19.64 $\pm$ 17.21 &  & 76.24 $\pm$ 1.85  & 49.32 $\pm$ 0.08 & 7.32 $\pm$ 0.35  & 48.94 $\pm$ 0.14  &  & 77.48 $\pm$ 3.6  & 49.51 $\pm$ 0.09 & 6.84 $\pm$ 0.92  & 48.83 $\pm$ 0.17 \\
\derpp   & 36.28 $\pm$ 21.72 & 23.65 $\pm$ 18.03 & 3.73 $\pm$ 3.5   & 22.23 $\pm$ 18.24 &  & 71.24 $\pm$ 18.09 & 45.1 $\pm$ 11.78 & 5.45 $\pm$ 1.36  & 43.93 $\pm$ 11.37 &  & 82.13 $\pm$ 7.11 & 49.44 $\pm$ 0.17 & 5.0 $\pm$ 1.63   & 48.44 $\pm$ 0.15 \\
\er      & 45.02 $\pm$ 24.73 & 23.77 $\pm$ 19.1  & 3.04 $\pm$ 2.47  & 24.28 $\pm$ 17.71 &  & 70.0 $\pm$ 7.37   & 48.94 $\pm$ 0.33 & 7.61 $\pm$ 1.45  & 47.55 $\pm$ 1.01  &  & 77.58 $\pm$ 1.77 & 49.32 $\pm$ 0.09 & 6.99 $\pm$ 0.47  & 48.86 $\pm$ 0.07 \\
\naive   & 59.99 $\pm$ 3.18  & 49.36 $\pm$ 0.42  & 10.72 $\pm$ 2.29 & 48.13 $\pm$ 1.34  &  & 57.55 $\pm$ 0.48  & 49.22 $\pm$ 0.11 & 12.91 $\pm$ 0.42 & 48.68 $\pm$ 0.19  &  & 59.91 $\pm$ 0.92 & 49.41 $\pm$ 0.04 & 12.34 $\pm$ 0.48 & 49.04 $\pm$ 0.12 \\
\restart & 59.05 $\pm$ 0.65  & 49.68 $\pm$ 0.01  & 12.97 $\pm$ 0.37 & 49.46 $\pm$ 0.02  &  & 58.12 $\pm$ 1.56  & 49.29 $\pm$ 0.09 & 12.98 $\pm$ 0.56 & 48.79 $\pm$ 0.16  &  & 59.1 $\pm$ 0.93  & 49.55 $\pm$ 0.07 & 13.23 $\pm$ 0.55 & 49.26 $\pm$ 0.1 
\end{tabular}

==> tables/clevr-shortcuts-results.tex <==
\begin{tabular}{llccccccccc}
                   &                         & \multicolumn{4}{c}{MNIST SHORTCUT}                                                                &  & \multicolumn{4}{c}{CLE4VR}                                                               \\
                   & model    & Class-IL($\vY$)       & Class-IL($\vC$)      & \textbf{OOD Acc ($\vY$)} & OOD Acc ($\vC$)   &  & Class-IL($\vY$)  & Class-IL($\vC$) & OOD Acc ($\vY$)   & OOD Acc ($\vC$)  \\
\multirow{8}{*}{\rotatebox{90}{$0\%$ \sc Supervision}}
                    & \offline   &  - $\pm$ - & - $\pm$ - & - $\pm$ -         & - $\pm$ -  &  & - $\pm$- & - $\pm$ -               & - $\pm$ -   & - $\pm$- \\
                   & \naive   &  59.99 $\pm$ 3.18  &  49.36 $\pm$ 0.42 & 10.72 $\pm$ 2.29         & 48.13 $\pm$ 1.34  &  & 44.87 $\pm$ 0.66 & 9.15 $\pm$ 1.22                & 25.0 $\pm$ 0.97   & 10.59 $\pm$ 1.16 \\
                   & \restart & 59.05 $\pm$ 0.65  & \bf 49.68 $\pm$ 0.01     & 12.97 $\pm$ 0.37         & 49.46 $\pm$ 0.02  &  & 39.07 $\pm$ 0.85 & 10.5 $\pm$ 1.43                & 11.11 $\pm$ 3.72  & 11.38 $\pm$ 1.0  \\
                   & \ewc     & 55.94 $\pm$ 8.9   & 45.62 $\pm$ 11.41 & 12.5 $\pm$ 1.44  & 45.45 $\pm$ 11.07 &  & 41.48 $\pm$ 7.09 & 8.32 $\pm$ 3.22  & 15.72 $\pm$ 8.38  & 8.73 $\pm$ 3.41  \\
                   & \lwf     & \bf 62.17 $\pm$ 1.79  & 49.11 $\pm$ 0.2   & 11.06 $\pm$ 1.2  & 48.48 $\pm$ 0.22  &  & 47.06 $\pm$ 0.83 & 6.61 $\pm$ 2.22  & 27.17 $\pm$ 2.83  & 7.58 $\pm$ 2.4   \\
                   & \er      & \bf 45.02 $\pm$ 24.73 & 23.77 $\pm$ 19.1     & 3.04 $\pm$ 2.47          & 24.28 $\pm$ 17.71 &  & 85.25 $\pm$ 0.28 & 10.26 $\pm$ 5.5                & 26.34 $\pm$ 3.52  & 11.26 $\pm$ 5.72 \\
                   & \der     & 41.36 $\pm$ 13.06 & 19.57 $\pm$ 17.41        & 7.88 $\pm$ 1.73          & 19.64 $\pm$ 17.21 &  & 77.74 $\pm$ 1.39 & 7.68 $\pm$ 2.81                &\bf 27.53 $\pm$ 2.72  & 8.42 $\pm$ 2.74  \\
                   & \derpp   & 36.28 $\pm$ 21.72 & 23.65 $\pm$ 18.03        & 3.73 $\pm$ 3.5           & 22.23 $\pm$ 18.24 &  &\bf 85.49 $\pm$ 0.15 & 11.07 $\pm$ 4.36               & 23.21 $\pm$ 1.78  &\bf 11.96 $\pm$ 4.49 \\
                   & \method  & 38.76 $\pm$ 26.25 & 24.08 $\pm$ 18.14        & 4.85 $\pm$ 2.02          & 23.61 $\pm$ 17.77 &  & 70.75 $\pm$ 5.74 & 8.45 $\pm$ 4.45                & 25.62 $\pm$ 2.3   & 8.95 $\pm$ 4.45  \\
                   &                         &                   &                                &                          &                   &  &                  &                                &                   &                  \\
\multirow{8}{*}{\rotatebox{90}{$1\%$ \sc Supervision}}
                    & \offline   &  - $\pm$ - & - $\pm$ - & - $\pm$ -         & - $\pm$ -  &  & - $\pm$- & - $\pm$ -               & - $\pm$ -   & - $\pm$- \\

                   & \naive   & 59.91 $\pm$ 0.92  & 49.41 $\pm$ 0.04         & 12.34 $\pm$ 0.48         & 49.04 $\pm$ 0.12  &  & 43.5 $\pm$ 2.69  & 19.96 $\pm$ 2.61               & 27.98 $\pm$ 11.41 & 19.17 $\pm$ 3.24 \\
                   & \restart & 59.1 $\pm$ 0.93   & 49.55 $\pm$ 0.07         & 13.23 $\pm$ 0.55         & 49.26 $\pm$ 0.1   &  & 39.95 $\pm$ 1.03 & 17.82 $\pm$ 0.13               & 14.76 $\pm$ 4.1   & 16.47 $\pm$ 0.19 \\
                   & \ewc     & 59.15 $\pm$ 1.48  & 49.51 $\pm$ 0.05  & 12.6 $\pm$ 0.83  & 49.08 $\pm$ 0.19  &  & 38.46 $\pm$ 6.45 & 17.21 $\pm$ 1.41 & 23.51 $\pm$ 8.57  & 16.0 $\pm$ 1.42  \\
                   & \lwf     & 55.84 $\pm$ 1.38  & 48.73 $\pm$ 0.13  & 12.5 $\pm$ 0.65  & 47.47 $\pm$ 0.16  &  & 41.91 $\pm$ 1.82 & 19.13 $\pm$ 2.96 & 29.04 $\pm$ 15.18 & 18.17 $\pm$ 3.52 \\
                   & \er      & 77.58 $\pm$ 1.77  & 49.32 $\pm$ 0.09         & 6.99 $\pm$ 0.47          & 48.86 $\pm$ 0.07  &  & 72.85 $\pm$ 4.86 & 20.52 $\pm$ 3.97               & 28.84 $\pm$ 9.89  & 19.4 $\pm$ 4.33  \\
                   & \der     & 77.48 $\pm$ 3.6   & 49.51 $\pm$ 0.09         & 6.84 $\pm$ 0.92          & 48.83 $\pm$ 0.17  &  & 73.29 $\pm$ 3.01 & 19.15 $\pm$ 1.98               & 24.88 $\pm$ 3.41  & 18.0 $\pm$ 2.33  \\
                   & \derpp   &\bf 82.13 $\pm$ 7.11  & 49.44 $\pm$ 0.17      & 5.0 $\pm$ 1.63           & 48.44 $\pm$ 0.15  &  &\bf 83.02 $\pm$ 1.13 & 20.92 $\pm$ 3.93             & 32.38 $\pm$ 12.13 & 20.12 $\pm$ 4.5  \\
                   & \method  & 70.72 $\pm$ 2.13  &\bf 80.23 $\pm$ 1.93      &\bf 57.05 $\pm$ 3.95      & \bf 76.8 $\pm$ 2.4&  &\bf 83.16 $\pm$ 0.48 & \bf 85.99 $\pm$ 2.85           & \bf 91.1 $\pm$ 1.52   & \bf 87.94 $\pm$ 3.45 \\
                   &                         &                   &                                &                          &                   &  &                  &                                &                   &                  \\
\multirow{8}{*}{\rotatebox{90}{$10\%$ \sc Supervision}} 
                    & \offline   &  - $\pm$ - & - $\pm$ - & - $\pm$ -         & - $\pm$ -  &  & - $\pm$- & - $\pm$ -               & - $\pm$ -   & - $\pm$- \\

                   & \naive   & 59.91 $\pm$ 0.92  & 49.41 $\pm$ 0.04         & 12.34 $\pm$ 0.48         & 49.04 $\pm$ 0.12  &  & 39.95 $\pm$ 1.64 & 17.86 $\pm$ 0.01               & 16.93 $\pm$ 3.57  & 16.56 $\pm$ 0.09 \\
                   & \restart & 59.1 $\pm$ 0.93   & 49.55 $\pm$ 0.07         & 13.23 $\pm$ 0.55         & 49.26 $\pm$ 0.1   &  & 39.15 $\pm$ 1.05 & 17.86 $\pm$ 0.01               & 13.69 $\pm$ 3.77  & 16.5 $\pm$ 0.09  \\
                   & \ewc     & 59.69 $\pm$ 0.86  & 49.56 $\pm$ 0.11  & 12.4 $\pm$ 0.29  & 49.2 $\pm$ 0.11   &  & 41.85 $\pm$ 1.8  & 17.85 $\pm$ 0.01 & 16.85 $\pm$ 4.34  & 16.61 $\pm$ 0.15 \\                                
                   & \lwf     & 58.04 $\pm$ 1.22  & 49.23 $\pm$ 0.1   & 12.62 $\pm$ 0.55 & 48.42 $\pm$ 0.15  &  & 39.53 $\pm$ 7.54 & 17.37 $\pm$ 3.9  & 44.86 $\pm$ 24.25 & 16.61 $\pm$ 3.32 \\
                   & \er      & 77.58 $\pm$ 1.77  & 49.32 $\pm$ 0.09         & 6.99 $\pm$ 0.47          & 48.86 $\pm$ 0.07  &  & 66.86 $\pm$ 8.39 & 18.27 $\pm$ 1.29               & 23.3 $\pm$ 4.03   & 16.98 $\pm$ 1.56 \\
                   & \der     & 77.48 $\pm$ 3.6   & 49.51 $\pm$ 0.09         & 6.84 $\pm$ 0.92          & 48.83 $\pm$ 0.17  &  & 75.06 $\pm$ 3.91 & 19.19 $\pm$ 2.02               & 26.1 $\pm$ 5.0    & 18.12 $\pm$ 2.43 \\
                   & \derpp   & \bf 82.13 $\pm$ 7.11  & 49.44 $\pm$ 0.17     & 5.0 $\pm$ 1.63           & 48.44 $\pm$ 0.15  &  & 81.25 $\pm$ 2.26 & 20.06 $\pm$ 3.95               & 28.39 $\pm$ 9.27  & 19.05 $\pm$ 4.56 \\
                   & \method  & 70.72 $\pm$ 2.13  & \bf 80.23 $\pm$ 1.93     & \bf 57.05 $\pm$ 3.95     & \bf 76.8 $\pm$ 2.4&  & \bf 85.24 $\pm$ 0.34 &\bf 87.96 $\pm$ 0.1         &\bf 91.85 $\pm$ 0.24  & \bf 89.85 $\pm$ 0.15
\end{tabular}

==> tables/clevr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{|c|r|r|}
\toprule
\multicolumn{1}{|l|}{sup=0.1} & \multicolumn{1}{l|}{CCIL}& \multicolumn{1}{l|}{CIL} \\ \midrule
\naive      & 17.86 $\pm$0.01             & 39.61  $\pm$ 2.55  \\
\restart    & 17.85 $\pm$0.02             &  39.75 $\pm$ 1.69  \\
\er         & 17.85  $\pm$ 0.01           & 58.11  $\pm$  5.06  \\
\der        & 17.85 $\pm$ 0.01            &  72.65  $\pm$  6.56  \\
\derpp      & 19.32  $\pm$ 2.56           & 67.13 $\pm$  8.90  \\
\method     & \textbf{87.76}  $\pm$ 0.15  & \textbf{84.10}  $\pm$ 0.86  \\
\methoder   & 87.19 $\pm$ 0.22            & 81.23 $\pm$  1.6 \\
\bottomrule
\end{tabular}




\begin{tabular}{|c|r|r|}
\hline
\multicolumn{1}{|l|}{sup=0} & \multicolumn{1}{l|}{CCIL}& \multicolumn{1}{l|}{CIL} \\ \hline
COOL    &$<$10 & 47.24  $\pm$ 4.99  \\ \hline
COOLER   &$<$10 & 81.23 $\pm$  1.6 \\ \hline
der     &$<$10  &  80.56  $\pm$  1.43 \\ \hline
derpp   &$<$10  & 	82.8 $\pm$ 1.17 \\ \hline
er      & $<$10  & \textbf{83.66}  $\pm$  0.28  \\ \hline
naive   &$<$10& 44.37  $\pm$ 0.20  \\ \hline
restart &$<$cool10  &  40.88 $\pm$ 0.45 \\ \hline
\end{tabular}

==> tables/mnist-sequential-setup.tex <==
\begin{tabular}{lccccccccc}
\toprule
                &  \sc Task $1$ &  \sc Task $2$ &  \sc Task $3$ &  \sc Task $4$ &  \sc Task $5$ &  \sc Task $6$ &  \sc Task $7$ &  \sc Task $8$ &  \sc Task $9$  \\ 
\textbf{Sums}   & $0$, $1$      & $2$, $3$      & $4$, $5$      & $6$, $7$      & $8$, $9$      & $10$, $11$    & $12$, $13$    & $14$, $15$    &  $16$, $17$   \\
\multicolumn{5}{*}{ \sc Concepts}  & $\MZero, \MOne$   & $\MZero, \MOne$ & $\MZero, \MOne$ & $\MZero, \MOne$ & $\MZero, \MOne$ & $\MZero, \MOne$ & $\MZero, \MOne$ \\
                                   &                   &  $\Two, \Three$ &  $\Two, \Three$              \\
                                   $\MFive$                                & $\MFive, \MSix, \MSeven$                 & $\MFive, \MSix, \MSeven, \MEight, \MNine$ \\
\bottomrule
\end{tabular}

==> tables/new-CBM-vs-NeSy.tex <==
% Please add the following required packages to your document preamble: 
% \usepackage{multirow}
\begin{tabular}{llcccccc}
& {\sc Strategy}& Task-IL($\vY$) ($\uparrow$)    & Task-IL($\vC$) ($\uparrow$)   & Class-IL($\vY$) ($\uparrow$)    & Class-IL($\vC$)($\uparrow$)    & BWT ($\uparrow$)& FWT ($\uparrow$) \\ \cmidrule{2-8}
\multirow{9}{*}{\rotatebox{90}{\sc CBM-$10\%$}} 
& \offline  & -       & -      &\underline{ 96.72 $\pm$ 0.17 }       &\underline{98.84 $\pm$ 0.11 }    &-         &-         \\

& \naive   & 27.51 $\pm$ 3.94          & 50.79 $\pm$ 1.67         & 11.71 $\pm$ 0.76         & 36.17 $\pm$ 2.64          & -91.07 $\pm$ 1.16          & 7.49 $\pm$ 0.27           \\
& \restart & 32.9 $\pm$ 2.1            & 43.07 $\pm$ 0.62         & 10.78 $\pm$ 0.06         & 29.65 $\pm$ 0.13          & -98.16 $\pm$ 0.12 & 7.24 $\pm$ 0.19           \\
& \lwf   & 55.69   $\pm$ 5.34       & 78.63  $\pm$2.54      &18.08  $\pm$  1.78      &  63.17 $\pm$ 4.38  &  \textbf{-18.51  $\pm$ 1.773}     &-4.70  $\pm$ 1.066       \\
& \ewc  & 38.34   $\pm$ 11.24         &52.14  $\pm$ 1.7      & 11.57 $\pm$ 0.63        & 37.40  $\pm$ 0.60     &-90.36 $\pm$ 0.8         &7.58  $\pm$ 0.40      \\
& \er      & 32.5 $\pm$ 3.2            & 67.74 $\pm$ 3.3          & 13.29 $\pm$ 0.4          & 43.48 $\pm$ 2.04          & -88.02 $\pm$ 0.73          & 13.37 $\pm$ 1.59          \\
% & \er\_ace (nostat) & 67.97 $\pm$ 0.0           & 88.83 $\pm$ 0.0          & 18.12 $\pm$ 0.0          & 71.35 $\pm$ 0.0           & -40.01 $\pm$ 0.1  & \textbf{33.55 $\pm$ 0.1}  \\
& \der     & 50.33 $\pm$ 3.39          & 73.09 $\pm$ 2.0          & 18.63 $\pm$ 2.5          & 53.14 $\pm$ 1.72          & -88.63 $\pm$ 2.86          & 15.66 $\pm$ 0.94          \\
& \derpp   & 48.89 $\pm$ 2.43          & 73.1 $\pm$ 4.48          & 18.17 $\pm$ 1.57         & 54.08 $\pm$ 2.97          & -89.2 $\pm$ 1.82           & 16.63 $\pm$ 1.75          \\
& \methoder   & \textbf{78.39 $\pm$ 3.77} & \textbf{90.4 $\pm$ 1.62} & \textbf{38.0 $\pm$ 1.88} & \textbf{78.05 $\pm$ 2.5}  & -68.25 $\pm$ 2.13          & \bf 29.04 $\pm$ 4.79          \\ \cmidrule{2-8}
\multirow{9}{*}{\rotatebox{90}{\sc DeepProbLog-$0\%$}}  
& \offline  & -         & -       & \underline{97.77 $\pm$ 0.20}          & \underline{98.87  $\pm$ 0.10}   &-         &-         \\
& \naive   & 7.61 $\pm$ 0.2            & 16.38 $\pm$ 0.96         & 6.88 $\pm$ 0.17          & 6.66 $\pm$ 0.38           & -63.09 $\pm$ 0.55          & 6.15 $\pm$ 0.15           \\
& \restart & 22.23 $\pm$ 0.8 & 11.6 $\pm$ 0.49 & 9.64 $\pm$ 0.25      & 0.18 $\pm$ 0.05   & -69.46 $\pm$ 1.93 & 6.91 $\pm$ 0.82   \\
& \lwf   &   11.03 $\pm$1.60       &  21.72 $\pm$8.33     &  6.78 $\pm$ 0.47      & 10.81 $\pm$ 4.62    &-71.179 $\pm$ 5.16        &18.259 $\pm$
0.2236       \\
& \ewc  &7.82 $\pm$  0.39               &18.26  $\pm$ 0.64          & 6.76 $\pm$ 0.41     & 7.83  $\pm$  0.56     &-62.853 $\pm$0.42      &6.107 $\pm$ 0.26     \\
& \er      & 81.24 $\pm$ 6.52          & 82.83 $\pm$ 5.13         & 44.29 $\pm$ 9.73         & 61.99 $\pm$ 8.64          & -48.3 $\pm$ 8.79           & 8.18 $\pm$ 4.07           \\
% & \er\_ace & 53.09 $\pm$ 31.87         & 55.66 $\pm$ 26.68        & 23.3 $\pm$ 19.87         & 35.1 $\pm$ 25.26          & -65.13 $\pm$ 16.27         & 13.08 $\pm$ 4.89          \\
& \der     & \bf 94.78 $\pm$ 3.2           & \bf 93.82 $\pm$ 3.04         & \bf 68.27 $\pm$ 9.4          & \bf 81.31 $\pm$ 6.87          & \bf -30.47 $\pm$ 8.45          & 44.46 $\pm$ 23.73         \\
& \derpp   & 93.47 $\pm$ 2.14          & 92.82 $\pm$ 2.89         & 62.22 $\pm$ 5.37         & 77.11 $\pm$ 4.16          & -34.75 $\pm$ 5.56          & 27.12 $\pm$ 5.18          \\
% & \method     & 96.21 $\pm$ 1.47          & 95.55 $\pm$ 0.71         & \textbf{72.12 $\pm$ 4.9} & \textbf{84.46 $\pm$ 3.16} & \textbf{-28.54 $\pm$ 5.51} & \textbf{83.65 $\pm$ 2.13} \\
& \methoder   & \textbf{96.64 $\pm$ 0.82} & \textbf{95.35 $\pm$ 0.4} & \bf 71.93 $\pm$ 2.89         & \bf 84.47 $\pm$ 1.85          & \bf -28.71 $\pm$ 3.16          & \bf 83.17 $\pm$ 0.88         \\
                                          \cmidrule{2-8}
\end{tabular}


==> tables/validation_parameters-sup0.tex <==
\begin{tabular}{lcccc}
\sc Strategy &  \MNISTAdd &\MNISTSeq&\CLEFVR   \\
\offline & lr=,;& lr=,;& lr=;\\
\naive & lr=;& lr=0.0001;& lr=0.0001;\\
\restart & lr=; ;& lr=0.001;& lr=0.0005; \\
\derpp & lr=, $\alpha=$& lr=0.001;  $\alpha=$& lr=0.001;  $\alpha=$;\\
\lwf & lr=,  $\alpha=$;& lr=0.0001,  $\alpha=$=;& lr=0.0001 $\alpha=$;\\
\ewc & lr=,  $\alpha=$, $\beta=$;& lr=0.0001,  $\alpha=$,$\beta=$;& lr=0.005,  $\alpha=$,$\beta=$;\\
\er & lr=;  $\alpha=$& lr=0.0005; $\alpha=$;& lr=0.0005;  $\alpha=$;\\
\der & lr=;  $\alpha=$;& lr=0.001;  $\alpha=$;& lr=0.001;  $\alpha=$;\\
\method & lr=; $\alpha=$;& lr=0.0005; $\alpha=$;& lr=0.001;  $\alpha=$;\\



\end{tabular}

==> tables/validation_parameters-sup10.tex <==
\begin{tabular}{lcccc}
\sc Strategy &  \MNISTAdd &\MNISTSeq&\CLEFVR   \\
\offline & lr=,;& lr=,;& lr=;\\
\naive & lr=;& lr=;& lr=0.0001;\\
\restart & lr=; ;& lr=;& lr=0.0005; \\
\derpp & lr=, $\alpha=$& lr=;  $\alpha=$& lr=0.001;  $\alpha=$;\\
\lwf & lr=,  $\alpha=$;& lr=,  $\alpha=$=;& lr=0.0001 $\alpha=$;\\
\ewc & lr=,  $\alpha=$, $\beta=$;& lr=,  $\alpha=$,$\beta=$;& lr=0.005,  $\alpha=$, $\beta=$;\\
\er & lr=;  $\alpha=$& lr=; $\alpha=$;& lr=0.0005;  $\alpha=$;\\
\der & lr=;  $\alpha=$;& lr=;  $\alpha=$;& lr=0.001;  $\alpha=$;\\
\method & lr=; $\alpha=$;& lr=; $\alpha=$;& lr=0.001;  $\alpha=$;\\



\end{tabular}

==> tables/validation_parameters-sup=1.tex <==
\begin{tabular}{lcccc}
\sc Strategy &  \MNISTAdd &\MNISTSeq&\CLEFVR   \\
\offline & lr=,;& lr=,;& lr=;\\
\naive & lr=;& lr=;& lr=0.0001;\\
\restart & lr=; ;& lr=;& lr=0.0005; \\
\derpp & lr=, $\alpha=$& lr=;  $\alpha=$& lr=0.001;  $\alpha=$;\\
\lwf & lr=,  $\alpha=$;& lr=,  $\alpha=$=;& lr=0.0001 $\alpha=$;\\
\ewc & lr=,  $\alpha=$, $\beta=$;& lr=,  $\alpha=$,$\beta=$;& lr=0.005,  $\alpha=$, $\beta=$;\\
\er & lr=;  $\alpha=$& lr=; $\alpha=$;& lr=0.0005;  $\alpha=$;\\
\der & lr=;  $\alpha=$;& lr=;  $\alpha=$;& lr=0.001;  $\alpha=$;\\
\method & lr=; $\alpha=$;& lr=; $\alpha=$;& lr=0.001;  $\alpha=$;\\



\end{tabular}
